Graph Neural Networks with Learnable Structural and Positional Representations

Graph neural networks (GNNs) have become the standard learning architectures for graphs. GNNs have been applied to numerous domains ranging from quantum chemistry, recommender systems to knowledge graphs and natural language processing. A major issue with arbitrary graphs is the absence of canonical positional information of nodes, which decreases the representation power of GNNs to distinguish e.g. isomorphic nodes and other graph symmetries. An approach to tackle this issue is to introduce Positional Encoding (PE) of nodes, and inject it into the input layer, like in Transformers. Possible graph PE are Laplacian eigenvectors. In this work, we propose to decouple structural and positional representations to make easy for the network to learn these two essential properties. We introduce a novel generic architecture which we call LSPE (Learnable Structural and Positional Encodings). We investigate several sparse and fully-connected (Transformer-like) GNNs, and observe a performance increase for molecular datasets, from 1.79% up to 64.14% when considering learnable PE for both GNN classes.

==> model_eqns_main.tex <==
\subsection{Sparse GNNs with \texttt{LSPE}}
\label{sec:sparse_gnns_lspe}
In this section, we augment two MP-GNN architectures with learnable positional representation, namely GatedGCN \citep{bresson2017residual} and PNA \citep{corso2020principal}.


\subsubsection{GatedGCN\texttt{-LSPE}}
\label{sec:gatedgcn_lspe}
GatedGCNs \citep{bresson2017residual} are sparse MP-GNNs equipped with a soft-attention mechanism that is able to learn adaptive edge gates to improve the message aggregation step of GCN networks \citep{kipf2017semi}.  We augment this model to develop GatedGCN\texttt{-LSPE}, defined as:
\begin{align}
    h^{\ell+1}, e^{\ell+1}, p^{\ell+1} &= \text{GatedGCN}\texttt{-LSPE}\Big(h^{\ell}, e^{\ell}, p^{\ell}\Big), \ h\in\mathbb{R}^{n\times d}, e\in\mathbb{R}^{E\times d}, p\in\mathbb{R}^{n\times d},\\
    \text{with} \ \ h_i^{\ell+1} &= h_i^{\ell} + \text{ReLU}\Big( \text{BN} \Big( A_1^{\ell} \left[ \!\!\begin{array}{c} h_i^\ell \\ p_i^\ell \\ \end{array} \!\!\right] + \sum_{j \in \mathcal{N}(i)} \eta_{ij}^{\ell} \odot A_2^{\ell} \left[ \!\!\begin{array}{c} h_j^\ell \\ p_j^\ell \\ \end{array} \!\!\right] \Big) \Big), \label{eqn:gatedcn_lspe_1}\\
e_{ij}^{\ell+1} &= e_{ij}^{\ell} + \text{ReLU}\big(\text{BN}\big(\hat{\eta}_{ij}^{\ell}\big)\big),\label{eqn:gatedgcn_lspe_2}\\
p_i^{\ell+1} &= p_i^{\ell} + \tanh \Big( C_1^{\ell}p_i^{\ell} + \sum_{j \in \mathcal{N}(i)} \eta_{ij}^{\ell} \odot C_2^{\ell}
  p_j^{\ell} \Big), \label{eqn:gatedgcn_lspe_3}\\
\text{and} \ \ \eta_{ij}^{\ell} &= \frac{\sigma\big(\hat{\eta}_{ij}^{\ell}\big)}{ \sum_{j' \in \mathcal{N}(i)} \sigma\big(\hat{\eta}_{ij'}^{\ell}\big) + \epsilon},\\[4pt]
\hat{\eta}_{ij}^{\ell} &= B_1^{\ell}h_i^{\ell} + B_2^{\ell}h_j^{\ell} + B_3^{\ell}e_{ij}^{\ell},
% p_i^{\ell+1} &= \frac{\hat{p}_i^{\ell+1}-\text{mean}_i\big(\hat{p}_i^{\ell+1}\big)}{\text{s.d.}_i\big(\hat{p}_i^{\ell+1}\big)},
\end{align}
where $h_i^{\ell}, e_{ij}^{\ell}, p_i^{\ell}, {\eta}_{ij}^{\ell}, \hat{\eta}_{ij}^{\ell} \in \mathbb{R}^{d}, A_1^{\ell}, A_2^{\ell} \in \mathbb{R}^{d \times 2d}$ and $B_1^{\ell}, B_2^{\ell}, B_3^{\ell}, C_1^{\ell}, C_2^{\ell} \in \mathbb{R}^{d \times d}$.


\subsubsection{PNA\texttt{-LSPE}}
\label{sec:pna_lspe}
PNA \citep{corso2020principal} is a sparse MP-GNN model which uses a combination of node aggregators to overcome the theoretical limitation of a single aggregator. We propose PNA\texttt{-LSPE} whose layer update equation is defined as:
\begin{align}
h^{\ell+1}, p^{\ell+1} &= \text{PNA}\texttt{-LSPE}\Big(h^{\ell}, e^0, p^{\ell}\Big), \ h\in\mathbb{R}^{n\times d}, e^0\in\mathbb{R}^{E\times d}, p\in\mathbb{R}^{n\times d},\\
\text{with} \ \ h_{i}^{\ell+1} &= h_{i}^{\ell} + \text{LReLU}\Big( \text{BN} \Big(U_h^{\ell}\left(\left[ \!\!\begin{array}{c} h_i^\ell \\ p_i^\ell \\ \end{array} \!\!\right], \bigoplus_{j \in \mathcal{N}(i)} M_h^{\ell}\left(\left[ \!\!\begin{array}{c} h_i^\ell \\ p_i^\ell \\ \end{array} \!\!\right], e_{ij}^0, \left[ \!\!\begin{array}{c} h_j^\ell \\ p_j^\ell \\ \end{array} \!\!\right]\right)\right)\Big)\Big), \label{eqn:pna_lspe_1}\\
p_{i}^{\ell+1} &= p_{i}^{\ell} + \tanh \Big(U_p^{\ell}\left(p_i^{\ell}, \bigoplus_{j \in \mathcal{N}(i)} M_p^{\ell}\Big(p_i^{\ell}, e_{ij}^0, p_j^{\ell}\Big)\right)\Big), \label{eqn:pna_lspe_2}\\
\text{and} \ \ \bigoplus \ &= \ \ {\left[\begin{array}{c}
I \\
S(D, \alpha=1) \\
S(D, \alpha=-1)
\end{array}\right]} \ \ \otimes \ \ {\left[\begin{array}{c}
\mu \\
\sigma \\
\max \\
\min
\end{array}\right]}, \label{eqn:pna_layer_agg_scalers}
% p_i^{(\ell+1)} &= \frac{\hat{p}_i^{(\ell+1)}-\text{mean}_i\Big(\hat{p}_i^{(\ell+1)}\Big)}{\text{s.d.}_i\Big(\hat{p}_i^{(\ell+1)}\Big)},
\end{align} 
where $\bigoplus$ is the principal aggregator designed in \citep{corso2020principal}, LReLU stands for LeakyReLU activation,
% the terms, \textit{say} $a$ and $b$, inside the small bracket with `\textbf{,}' operator \textit{i.e.,} $(a \ \textbf{,} \ b)$, are concatenated; similarly, the terms inside the square bracket $[ \ ]$ are concatenated;
amd $U_h^{\ell}, U_p^{\ell}, M_h^{\ell}$ and $M_p^{\ell}$ are linear layers (or multi-layer perceptrons) with learnable parameters.


\subsection{Transformer GNNs with \texttt{LSPE}}
\label{sec:transformer_lspe}

The recently developed SAN \citep{kreuzer2021rethinking}, GraphiT \citep{mialon2021graphit} and Graphormer \citep{ying2021transformers} are promising full-graph operable Transformers incorporating several methods to encode positional and structural features into the network. In the next sections, we expand these Transformer-based networks with the proposed \texttt{-LSPE} architecture to further improve their performance. 


\subsubsection{SAN\texttt{-LSPE}}
\label{sec:san_lspe}
Like Transformers, Spectral Attention Networks (SAN) \citep{kreuzer2021rethinking} operate on full graphs although the network separates the parameters coming from existing edges and non-existing edges in the graph. Furthemore, the contribution of attentions from existing and non-existing edges are weighted by an additive positive scalar $\gamma$, which can be tuned for different tasks. SAN also considers a Learnable Positional Encoding (LPE) module which takes in Laplacian eigenvectors and transforms them into a fixed size PE with a self-attention encoder. This PE is then used in the main architecture in a manner similar to MP-GNNs\texttt{-PE} as defined in Eq. (\ref{eqn:mpgnn-pe-input}). We propose to extend SAN by replacing the LPE module with the \texttt{LSPE} architecture proposed in Section \ref{sec:generic_formulation} where positional representation is learned in line with structural embedding at each GNN layer:
\begin{align}
h^{\ell+1}, p^{\ell+1} &= \text{SAN}\texttt{-LSPE}\Big(h^{\ell}, e^0, p^{\ell}\Big), \ h\in\mathbb{R}^{n\times d}, e^0\in\mathbb{R}^{n\times n\times d}, p\in\mathbb{R}^{n\times d},\label{eqn:san_lspe_1}\\
\text{with} \ \ h_{i}^{\ell+1}&=\text{BN}\left(\bar{h}_{i}^{\ell+1}+  W_{2}^{\ell}\ \text{ReLU}\left( W_{1}^{\ell}\ \bar{h}_{i}^{\ell+1} \right) \right)\in\mathbb{R}^{d}\\
\bar{h}_{i}^{\ell+1}&=\text{BN}\left(h_{i}^{\ell}+\hat{h}_{i}^{\ell+1}\right)\in\mathbb{R}^{d},\label{eqn:san_lspe_2}
\end{align}
\begin{eqnarray}
\hat{{h}}_{i}^{\ell+1}= O^{\ell}\Big(\bigparallel_{k=1}^{H}\sum_{j \in \mathcal{V}} \frac{w_{ij}^{k, \ell}}{\sum_{j' \in \mathcal{V}} w_{ij'}^{k, \ell}} \ v_j^{k,\ell} \Big)\in\mathbb{R}^{d},\label{eqn:san_lspe_3}
\end{eqnarray}
\begin{eqnarray}
w_{ij}^{k,\ell}=\left\{\begin{array}{ll}
\frac{1}{1+\gamma} \cdot \text{exp}(A_{ij}^{k,\ell}) & \textrm{ if } ij\in E  \\
\frac{\gamma}{1+\gamma} \cdot \text{exp}(\bar{A}_{ij}^{k,\ell}) & \textrm{ if } ij\not\in E \\
\end{array}\right.,\label{eqn:san_lspe_3a}
\end{eqnarray}
\begin{eqnarray}
\left\{
\begin{array}{ll}
A_{ij}^{k,\ell}={q_i^{k,\ell}}^T \textrm{diag}(c_{ij}^{k,\ell}) k_j^{k,\ell} / \sqrt{d_k}\in\mathbb{R} & \textrm{ if } ij\in E \\
\bar{A}_{ij}^{k,\ell}=\bar{q}_i{{}^{k,\ell}}^T\textrm{diag}({\bar{c}}_{ij}^{k,\ell}) {\bar{k}}_j^{k,\ell} / \sqrt{d_k}\in\mathbb{R} & \textrm{ if } ij\not\in E 
\end{array}
\right.
\end{eqnarray}
\begin{eqnarray}
Q^{k,\ell} &\!=\! \left[ \!\!\begin{array}{c} h^\ell \\ p^\ell \\ \end{array} \!\!\right] W_{Q}^{k,\ell},\
K^{k,\ell} \!=\! \left[ \!\!\begin{array}{c} h^\ell \\ p^\ell \\ \end{array} \!\!\right] W_{K}^{k,\ell},\
V^{k,\ell} \!=\! \left[ \!\!\begin{array}{c} h^\ell \\ p^\ell \\ \end{array} \!\!\right] W_{V}^{k,\ell}\in\mathbb{R}^{n\times d_k}\\
\bar{Q}^{k,\ell} &\!=\! \left[ \!\!\begin{array}{c} h^\ell \\ p^\ell \\ \end{array} \!\!\right] \bar{W}_{Q}^{k,\ell},\
\bar{K}^{k,\ell} \!=\! \left[ \!\!\begin{array}{c} h^\ell \\ p^\ell \\ \end{array} \!\!\right] \bar{W}_{K}^{k,\ell},\
\bar{V}^{k,\ell} \!=\! \left[ \!\!\begin{array}{c} h^\ell \\ p^\ell \\ \end{array} \!\!\right] \bar{W}_{V}^{k,\ell}\in\mathbb{R}^{n\times d_k}
\end{eqnarray}
\begin{eqnarray}
C^{k,0} \!=\! e^0 W_{e}^{k}, \ \bar{C}^{k,0} \!=\! e^0 \bar{W}_{e}^{k}\in\mathbb{R}^{n\times n\times d_k} 
\end{eqnarray}
\begin{align}
\text{and} \ \ {p}_{i}^{\ell+1}&= p_i^{\ell} + \tanh \Big( {O}_{p}^{\ell} \Big( \bigparallel_{k=1}^{H}\sum_{j \in \mathcal{V}} \frac{w_{p,i j}^{k, \ell}}{\sum_{j' \in \mathcal{V}} w_{p,i j'}^{k, \ell}} v_{p,j}^{k,\ell}\Big)\Big)\in\mathbb{R}^d,\label{eqn:san_lspe_5}
\end{align}
\begin{eqnarray}
w_{p,ij}^{k,\ell}=\left\{\begin{array}{ll}
\frac{1}{1+\gamma} \cdot \text{exp}(A_{p,ij}^{k,\ell}) & \textrm{ if } ij\in E  \\
\frac{\gamma}{1+\gamma} \cdot \text{exp}(\bar{A}_{p,ij}^{k,\ell}) & \textrm{ if } ij\not\in E \\
\end{array}\right.,\label{eqn:san_lspe_3a_p}
\end{eqnarray}
\begin{eqnarray}
\left\{
\begin{array}{ll}
A_{p,ij}^{k,\ell}={q_{p,i}^{k,\ell}}^T \textrm{diag}(c_{p,ij}^{k,\ell}) k_{p,j}^{k,\ell} / \sqrt{d_k}\in\mathbb{R} & \textrm{ if } ij\in E \\
\bar{A}_{p,ij}^{k,\ell}=\bar{q}_{p,i}{{}^{k,\ell}}^T\textrm{diag}({\bar{c}}_{p,ij}^{k,\ell}) {\bar{k}}_{p,j}^{k,\ell} / \sqrt{d_k}\in\mathbb{R} & \textrm{ if } ij\not\in E 
\end{array}
\right.
\end{eqnarray}
\begin{eqnarray}
Q_p^{k,\ell} &\!=\! p^\ell W_{p,Q}^{k,\ell},\
K_p^{k,\ell} \!=\! p^\ell W_{p,K}^{k,\ell},\
V_p^{k,\ell} \!=\! p^\ell W_{p,V}^{k,\ell}\in\mathbb{R}^{n\times d_k}\\
\bar{Q}_p^{k,\ell} &\!=\! p^\ell \bar{W}_{p,Q}^{k,\ell},\
\bar{K}_p^{k,\ell} \!=\! p^\ell \bar{W}_{p,K}^{k,\ell},\
\bar{V}_p^{k,\ell} \!=\! p^\ell \bar{W}_{p,V}^{k,\ell}\in\mathbb{R}^{n\times d_k}
\end{eqnarray}
\begin{eqnarray}
C_p^{k,0} \!=\! e^0 W_{p,e}^{k}, \ \bar{C}_p^{k,0} \!=\! e^0 \bar{W}_{p,e}^{k}\in\mathbb{R}^{n\times n\times d_k} 
\end{eqnarray}
where $W_1^{\ell}, W_2^{\ell} \in \mathbb{R}^{d \times d}$, $O^{\ell}, O_p^{\ell} \in \mathbb{R}^{d \times d}$, $W_Q^{k,\ell},W_K^{k,\ell},W_V^{k,\ell},\bar{W}_Q^{k,\ell},\bar{W}_K^{k,\ell},\bar{W}_V^{k,\ell} \in \mathbb{R}^{2d \times d_k}$, $W_{p,Q}^{k,\ell},W_{p,K}^{k,\ell},W_{p,V}^{k,\ell},\bar{W}_{p,Q}^{k,\ell},\bar{W}_{p,K}^{k,\ell},\bar{W}_{p,V}^{k,\ell} \in \mathbb{R}^{d \times d_k}$, $W_{e}^{k}, \bar{W}_{e}^{k}, W_{p,e}^{k}, \bar{W}_{p,e}^{k}\in \mathbb{R}^{d \times d_k}$, and $d_k = d/H$ is the dimension of the $k^{th}$ head for a total of $H$ heads. BN denotes the standard Batch Normalization \citep{ioffe2015batch}. Finally, we make the balance scalar parameter $\gamma\geq 0$ learnable (also clipping its range in $[0,1]$) differently from \citep{kreuzer2021rethinking} where its optimal value is computed by grid search. 


\subsubsection{GraphiT\texttt{-LSPE}}
\label{sec:graphit_lspe}

Similarly to SAN, GraphiT \citep{mialon2021graphit} is a full-graph operable Transformer GNN which makes use of the diffusion distance to capture short-range and long-range interactions between nodes depending of the graph topology. This pairwise diffusion distance is used as a multiplicative weight to adapt the weight scores to the closeness or farness of the nodes. For example, if two nodes are close on the graph, them the diffusion distance $K_{ij}$ will have a value close to one, and when the two nodes are far away then the value of $K_{ij}$ will be small. 

Unlike SAN, the GraphiT model does not consider separate parameters for existing and non-existing edges for a graph. However, following \citep{kreuzer2021rethinking} and our experiments,  separating the parameters for each type of edges showed to improve the performance. Therefore, we augment the original GraphiT architecture with learnable positional features and use two sets of parameters for the edges and the complementary edges to define GraphiT\texttt{-LSPE}. The GraphiT\texttt{-LSPE} model uses the same update equation as SAN\texttt{-LSPE} except for the weight score which are re-defined to introduce the diffusion kernel:
\begin{eqnarray}
w_{ij}^{k,\ell}=\left\{\begin{array}{ll}
K_{ij} \cdot \text{exp}(A_{ij}^{k,\ell}) & \textrm{ if } ij\in E  \\
K_{ij} \cdot \text{exp}(\bar{A}_{ij}^{k,\ell}) & \textrm{ if } ij\not\in E \\
\end{array}\right..\label{eqn:san_lspe_3a_graphit}
\end{eqnarray}
Following \citep{mialon2021graphit}, the diffusion distance is chosen to be the $p$-step random walk kernel defined as $K = (\textrm{I}_n - \beta \Delta)^p \in \mathbb{R}^{n \times n}$ where $\textrm{I}_n, \Delta \in \mathbb{R}^{n \times n}$ is the identity matrix and the graph Laplacian matrix respectively. Hyper-parameter $\beta$ controls the amount of diffusion with value between $[0.25,0.50]$. 


